Report on Progress in Physics: Observation of the Breit-Wheeler Process and Vacuum Birefringence in Heavy-Ion Collisions

This Report reviews the effort over several decades to observe the linear Breit-Wheeler process ($\gamma\gamma \rightarrow e^+e^-$) and vacuum birefringence in high-energy particle and heavy-ion collider experiment. This Report, motivated by STAR's recent observations, attempts to summarize the key issues related to the interpretation of polarized $\gamma\gamma \rightarrow l^+l^-$ measurements in high-energy experiments. To that end, we start by reviewing the historical context and essential theoretical developments, before focusing on the decades of progress made in high-energy collider experiments. Special attention is given to the evolution in experimental approaches in response to various challenges and the demanding detector capabilities required to unambiguously identify the linear Breit-Wheeler process and to detect the signatures of vacuum birefringence. We close the report with a discussion, followed by a look at near-future opportunities for utilizing these discoveries and for testing QED in previously unexplored regimes.

==> section_photon_virtuality.tex <==
\subsubsection{ Lowest-order QED }
The pair creation in lowest-order two photon interaction can be depicted as a process with two Feynman diagrams contributing, as shown in Fig.2 of Ref.~\cite{PhysRevA.51.1874}. There is an approximation commonly used for describing events: that of external fields generated by nuclei that are undeflected by the collision and travel along straight-line trajectories. 
Following the derivation of Ref.~\cite{PhysRevA.51.1874,PhysRevA.55.396}, the cross section for pair production of leptons is given by
\begin{equation}
\label{eq:cross_section_pair}
    \sigma = \int d^{2}b \frac{d^{6}P(\vec{b})}{d^{3}p_{+}d^{3}p_{-}} = \int d^{2}q \frac{d^{6}P(\vec{q})}{d^{3}p_{+}d^{3}p_{-}} \int d^{2}b e^{i {\vec{q}} \cdot  {\vec{b}}},
\end{equation}
and the differential probability $\frac{d^{6}P(\vec{q})}{d^{3}p_{+}d^{3}p_{-}}$ in QED at the lowest order is
\begin{align}
    \label{equation_differential_probability}
    \begin{split}
        \frac{d^{6}P(\vec{q})}{d^{3}p_{+}d^{3}p_{-}} & = (Z\alpha_{em})^{4} \frac{4}{\beta^{2}} \frac{1}{(2\pi)^{6}2\epsilon_{+}2\epsilon_{-}} \\ 
        & \times \int d^{2}q_{1} \frac{F(N_{0})F(N_{1})F(N_{3})F(N_{4})}{N_{0}N_{1}N_{3}N_{4}} \\
        % & \times []^{-1} \\
        & \times {\rm{Tr}}\bigg\{(\slashed{p}_{-}+m)\bigg[N_{2D}^{-1}\slashed{u}_{1} (\slashed{p}_{-} - \slashed{q}_{1} + m)\slashed{u}_{2} \\
        & + N_{2X}^{-1}\slashed{u}_{2}(\slashed{q}_{1} - \slashed{p}_{+} +m)\slashed{u}_{1}\bigg] (\slashed{p}_{+}-m) \\
        & \times \bigg[N_{5D}^{-1}\slashed{u}_{2} (\slashed{p}_{-} - \slashed{q}_{1} - \slashed{q} + m)\slashed{u}_{1} \\ 
        & + N_{5X}^{-1} \slashed{u}_{1} (\slashed{q}_{1} + \slashed{q} - \slashed{p}_{+} + m)\slashed{u}_{2}\bigg] \bigg\},
    \end{split}
\end{align}
with
\begin{align}
    \label{equation_N}
    \begin{split}
        N_{0} & = -q_{1}^{2},  \\
        N_{1} & = -[q_{1} - (p_{+}+p_{-})]^{2},\\
        N_{3} & = -(q_{1}+q)^{2}, \\
        N_{4} & = -[q+(q_{1} - p_{+} - p_{-})]^{2}, \\
        N_{2D} & = -(q_{1} - p_{-})^{2} + m^{2},\\
        N_{2X} & = -(q_{1} - p_{+})^{2} + m^{2}, \\
        N_{5D} & = -(q_{1} + q - p_{-})^{2} + m^{2},\\
        N_{5X} & = -(q_{1} + q  - p_{+})^{2} + m^{2},
    \end{split}
\end{align}
where $b$ is the nucleus-nucleus impact parameter, $F(...)$ is the nuclear electromagnetic form factor, $p_{+}$ and $p_{-}$ are the momenta of the created leptons, the longitudinal components of $q_{1}$ are given by $q_{10} = \frac{1}{2}[(\epsilon_{+} + \epsilon_{-}) + \beta(p_{+z}+p_{-z})]$, $q_{1z} = q_{10}/ \beta$, $\epsilon_{+}$ and $\epsilon_{-}$ are the energies of the produced leptons, and $m$ is the mass of the lepton. 
In order to compute results at all impact parameters, where in general no simple analytical form is available, the multi-dimensional integration is performed with the VEGAS Monte Carlo integration routine~\cite{peterlepageNewAlgorithmAdaptive1978}. 

The nuclear electromagnetic form factor can be obtained via the Fourier transform of the charge distribution as
    \begin{equation}
    \label{eq:formFactor2}
    F(k^{2}) = \int d^{3}re^{ik.r}\rho_{A}(r).
    \end{equation}

In this Article, we assume that the charges in the target and projectile nuclei are distributed according to the Woods-Saxon distribution ~\cite{doi.10.1103/PhysRev.95.577} without any fluctuations or point-like structure as
    \begin{equation}
    \label{eq:charge_density2}
    \rho_{A}(r)=\frac{\rho^{0}}{1+\exp[(r-R_{\rm{WS}})/d]}
    %\label{equation17}
    \end{equation}
where the radius $R$ (Au: 6.38 fm) and skin depth $d$ (Au: 0.535 fm) are based on fits to low energy electron scattering data such that all deformations are assumed to be higher order and are ignored~\cite{doi.10.1016/0092-640X(87)90013-1}, and $\rho^{0}$ is the density at the center of nucleus. The Fourier transform of the Woods-Saxon distribution does not have an analytic form, it was computed numerically for the following calculations.  

The EPA is used when deriving the cross section for pair production in Eq.~\eqref{eq:cross_section_pair}. According to the EPA, the number spectrum of photons with energy $\omega$~\cite{Krauss:1997vr} manifest by the field of a single nucleus is:
    \begin{equation}
    \label{eq:photon_density2}
    n(\omega) = \frac{(Ze)^{2}}{\pi\omega}\int_{0}^{\infty}\frac{d^{2}k_{\perp}}{(2\pi)^{2}}\left[\frac{F\left(\left(\frac{\omega}{\gamma}\right)^{2}+\overrightarrow{k}_{\perp}^{2}\right)}{\left(\frac{\omega}{\gamma}\right)^{2}+\overrightarrow{k}_{\perp}^{2}}\right]^{2}\overrightarrow{k}_{\perp}^{2},
    \end{equation}
where $Z$ is the nuclear charge number, $\gamma$ is the Lorentz factor, $\overrightarrow{k}_{\perp}$ is the photon transverse momentum, and $F\left(\left(\frac{\omega}{\gamma}\right)^{2}+\overrightarrow{k}_{\perp}^{2}\right)$ is the nuclear electromagnetic form factor.

\subsubsection{Photon Virtuality and a Criterion for the Breit-Wheeler Process}
\label{sec:Virtuality}
It is often considered that the transverse momentum of the photons in UPC is related to the transverse dimensions of the nuclei and the virtuality of the photons as discussed in the previous section. 
This has been used as an argument~\cite{PhysRevC.70.031902,doi.10.1016/j.cpc.2016.10.016,Esnault_2021,Zhao:2021ynd} that the $e^+e^-$ pair production from UPC is not the Breit-Wheeler process despite the original proposal in the Breit-Wheeler paper~\cite{PhysRev.46.1087}. In this section, we follow Ref.~\cite{PhysRevC.47.2308} using the S-Matrix derivation to illustrate the approximation which results in the EPA and propose a criterion for defining the Breit-Wheeler process in relativistic heavy-ion collisions. 

Since the Coulomb field is a pure electric field, the Lorentz boost does not change the fact that real photons cannot be generated by the field itself. 
The resulting quantization as photons from the Poynting Vector would have the form as shown in~\cref{eq:photon_density} with a spacelike Lorentz vector and a "negative squared mass" of $-((\omega/\gamma)^2+k_{\perp}^2)$. 
It was argued that if one were to define the process in UPC as the Breit-Wheeler process, the virtuality would simply have to be ignored. In fact, this is not the case. In fact, setting this term to zero would result in infrared divergence of the photon flux. 
Equation 25 in Ref.~\cite{PhysRevC.47.2308} shows the approximation required for the conserved transition current to behave as real photon interactions in the S-Matrix. The requirement in the center-mass-frame of the heavy-ion collision is that both photons satisfy the following condition: 
    \begin{equation}
    \label{equation_BW_criterion1}
    \omega/\gamma\, \lesssim \, k_{\perp}\, <<\, \omega     \end{equation}

With this criterion and subsequent omission of the higher order second and third terms of the order of $1/\gamma^2$, the vertex function of the two-photon process in relativistic heavy-ion collisions in Eq. 28 of Ref.~\cite{PhysRevC.47.2308} would be identical to that of the real-photon interaction in Eq. 19 of Ref.\cite{PhysRevC.47.2308}. 
The interpretation is therefore that the single photon flux of the virtual states from the Lorentz boosted field is given by \cref{eq:photon_density} and that the interaction is only relevant for (or behaves as) photons with real-photon states characterized by energy of $\omega$ and transverse momentum of $k_{\perp}$, validating the implementation of the so-called photon Wigner function (PWF)~\cite{PhysRevD.102.094013,PhysRevD.101.034015,KLUSEKGAWENDA2021136114,PhysRevD.104.056011}. 
Since the form factor (field strength) in the photon flux limits the photon transverse momentum to be $k_{\perp} \lesssim 1/R$, this puts a further constraint on the available phase space for the photons that may participate in the Breit-Wheeler process: 
    \begin{equation}
    \label{equation_BW_criterion2}
    \omega/\gamma\, \lesssim\, k_{\perp}\, \lesssim\, 1/R\, \ll\, \omega     \end{equation}
With decreasing beam energy ($\gamma$) in the same kinematic acceptance, the phase space for the Breit-Wheeler process decreases and we would expect that the photons outside this valid range ($k_{\perp}\lesssim\omega/\gamma$) to contribute substantially to the interaction cross section at low beam energy. 

==> section_v.tex <==
The first heavy-ion collisions experiments were envisaged as a tool for studying nuclear matter in a previously unexplored regime. Unlike high-energy $e^++e^-$ and hadron colliders, heavy-ion collisions produce a relatively larger and hotter system capable of vaporizing the normal matter within nuclei -- reaching temperatures of $\sim4$ trillion Kelvin\cite{}. The first manifestation of heavy-ion collisions were provided by accelerators with a fixed-target configuration such as the Super Proton Synchrotron, which was capable of colliding sulfer ions with fixed targets of Al, Pd, and Au~\cite{}. Despite the focus on nuclear physics, heavy-ion collisions have been understood as a unique tool for studying QED in unique regimes for a century~\cite{WW_and_TOLL}, with significant interest in the last 40 years~\cite{eichlerTheoryRelativisticIonatom1990,baurMultipleElectronpositronPair1990,baltzCoulombCorrectionsProduction2001}.

In the year 2000, the Relativistic Heavy Ion Collider (RHIC) began operation and ushered in a new era of high-energy nuclear physics with ultra-relativistic Au beams providing heavy-ion collisions with a center-of-mass energy per nucleon pair $(\sqrt{s_{NN}})$ two orders of magnitude larger than the proton mass $(\sim 1 {\rm GeV})$. The payoff from this next-generation facility was almost immediate, with all four RHIC experiments reporting observation of a new state of matter by 2004: The Quark Gluon Plasma (QGP)~\cite{}.   

% Figure of the 4 experiments at RHIC

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/star_2004_ee_dm.pdf}
    \includegraphics[width=0.48\textwidth]{figures/star_2004_ee.pdf}
    \caption{ STAR measurement of the invariant mass (left) and transverse momentum (right) distribution of photo-produced $e^+e^-$. The  data points are compared with predictions from the EPA (solid histogram) and lowest-order QED (dashed histogram) calculations. The error bars include both statistical and systematic errors.}
    \label{fig:star_2004}
\end{figure}


\subsubsection{Early Measurements}
Right from the start, the two ``large'' experiments at RHIC (STAR and PHENIX) studied the electromagnetic production of $e^+e^-$ from the fields of the colliding ultra-relativistic Au nuclei~\cite{adamsProductionPairsAccompanied2004,afanasievPhotoproductionPsHigh2009a}. The STAR Collaboration produced the first measurement of this kind from Au+Au collisions collected in the year 2001. At that time events were selected with a minimum-bias trigger condition -- meant to select Au+Au collisions from central (head-on, $b\approx0$) to peripheral (glancing $b\approx 2R_{\rm Au}$). Such a minimum-bias trigger is ideal for selecting event with nuclear overlap and is commonly used (with varying implementations) across all existing heavy-ion collider experiments. 

However, such a trigger condition is not ideal for selecting electromagnetically produced $e^+e^-$, since those kinds of events are nearly empty, except for the two charged tracks left by the $e^+$ and $e^-$. For this reason only 52 candidate events out of the 2001 data set, consisting of $\sim$800\,000 minimum-bias events, survived the additional selection criteria imposed to identify electromagnetically produced $e^+e^-$. Figure~\ref{fig:star_2004} shows the observed differential cross section, in terms of the pair invariant mass (left) and the pair transverse momentum (right). The data are found to exhibit reasonable agreement with the theoretical calculations based on the traditional EPA approach (solid line) and numerical lowest-order QED calculations (dotted line) shown for comparison. 

While the two theoretical calculations were nearly identical in terms of the predicted cross section, there was one crucial difference visible in the predicted pair transverse momentum distribution. The traditional EPA predicted that the cross section should continue to rise toward pair momentum of zero while the QED calculation predicted a significant depletion of the differential cross section for pair momentum below 20 MeV.
Even given the large statistical uncertainties of the measurement due to the small sample of only 52 pairs, the measured transverse momentum distribution clearly favored the numerical lowest order QED calculation. It is at this point crucial to recognize that the theoretical developments discussed in Section~\ref{sec:flux}B came more than a decade after this early result from STAR. At the time, the discrepancy between the traditional EPA and QED calculations were interpreted as arising from the effect of photon virtuality~\cite{adamsProductionPairsAccompanied2004}:
\begin{quote}
    The main difference between this calculation and the EPA approach is that the QED calculation includes photon virtuality.
\end{quote}
As discussed in Section~\ref{sec:photon_sources_hic}, this is now understood to be an incorrect statement, with the difference resulting primarily from the impact parameter dependence of the process (included in the QED calculation but not in the traditional EPA) -- not from photon virtuality\cite{zha:2018tlq}. Furthermore, this interpretation was oft-repeated e.g. in a highly-cited review paper~\cite{bertulaniPhysicsUltraPeripheralNuclear2005} on the subject that followed closely after the STAR measurement was published:
\begin{quote}
    These photons are almost real, with virtuality $-q^2 < (\hbar/R_A)^2$. Except for the production of $e^+e^-$ pairs, the photons can usually be treated as real photons.
\end{quote}
This view became commonplace in the literature, with similar statements appearing in many papers over the next decade and a half~\cite{}. 
However, as we will discuss in the next subsections, experimental progress\footnote{and theoretical progress, as discussed in Section~\ref{sec:flux}} began to challenge this view. 

\subsubsection{Experimental Approaches, Detector Requirements, and Limitations}

Over the next decade and a half between $\sim$2005 and 2020



\cite{abbasCharmoniumPairPhotoproduction2013}
\newpage
